Standalone FPGA-Based QAOA Emulator for Weighted-MaxCut on Embedded Devices

Quantum computing QC emulation is crucial for advancing QC applications, especially given the scalability constraints of current devices. FPGA-based designs offer an efficient and scalable alternative to traditional large-scale platforms, but most are tightly integrated with high-performance systems, limiting their use in mobile and edge environments. This study introduces a compact, standalone FPGA-based QC emulator designed for embedded systems, leveraging the Quantum Approximate Optimization Algorithm (QAOA) to solve the Weighted-MaxCut problem. By restructuring QAOA operations for hardware compatibility, the proposed design reduces time complexity from O(N^2) to O(N), where N equals 2^n for n qubits. This reduction, coupled with a pipeline architecture, significantly minimizes resource consumption, enabling support for up to nine qubits on mid-tier FPGAs, roughly three times more than comparable designs. Additionally, the emulator achieved energy savings ranging from 1.53 times for two-qubit configurations to up to 852 times for nine-qubit configurations, compared to software-based QAOA on embedded processors. These results highlight the practical scalability and resource efficiency of the proposed design, providing a robust foundation for QC emulation in resource-constrained edge devices.

==> tables/pro_optlist_split.tex <==

\footnotesize

\renewcommand{\arraystretch}{1.3} %셀 세로 여백 조절
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c}
\toprule
Operation               		& \multirow{2}{*}{Operation Module} 		& \multirow{2}{*}{Power\tnote{*}}     	& Speed-up         			\\ 
Type &&&compared to SW \\ \toprule
\rowcolor[HTML]{EBEBEB} 
%Add/Sub               		& florian-minimum               	& 0.37       		& \textbf{5.77$\times$} faster                  \\ \midrule
Add/Sub               		& Florian-Pro\_essential             & 0.37       		& \textbf{5.77$\times$} faster                  \\ \midrule
\multirow{2}{*}{Mult} 	& $mult\_basic$                    	& 0.038      		& \textbf{3.05$\times$} faster                  \\
                      			& $mult\_fullhw$                   	& 0.058      		& \textbf{7.66$\times$} faster                  \\ \midrule
\multirow{4}{*}{Div}  	& $div\_basic$ (w/ $mult\_basic$)  	& 0.0074     		& \multirow{2}{*}{\textbf{1.20$\times$} faster} \\
                      			& $div\_basic$ (w/o   $mult\_basic$) & 0.038      		&                        				\\
                      			& $div\_fullhw$                   		& 0.093      		& \textbf{5.81$\times$} faster                  \\
                     		 	& $div\_doublehw$                 	& 0.15       		& \textbf{8.03$\times$} faster                  \\ \midrule
\multirow{2}{*}{Conv} 	& $conv\_ftoi$                    		& 0.018      		& \textbf{1.36$\times$} faster                  \\ \cline{2-4} 
                      			& $conv\_itof$                    		& 0.026      		& \textbf{2.25$\times$} faster                  \\ \midrule
\multirow{3}{*}{Comp} 	& $comp\_eq$                      	& 0.038 			& \textbf{1.37$\times$} faster                  \\ \cline{2-4} 
                      			& $comp\_size$ (w/ $comp\_eq$)  	& 0.022 			& \multirow{2}{*}{\textbf{1.71$\times$} faster} \\
                      			& $comp\_size$ (w/o   $comp\_eq$)	& 0.049 			&                        			\\ \bottomrule
\multicolumn{4}{r}{$*$ normalized based on power consumption of a single ORCA core} 
\end{tabular}%
}




==> tables/resource_fpga_original.tex <==

\footnotesize

\begin{tabular}{c|cc|c|cc}
&\multicolumn{2}{c|}{Rocket} &ORCA &\multicolumn{2}{c}{Florian-}\\ 
&Core &FPU &core &FPU &Arbiter\\\midrule
LUTs &11711 &5456 &3230 &1546 &144 \\
FFs &6653 &1775 &3056 &558 &89 \\ \midrule
\end{tabular}


